The Vector Balancing Constant for Zonotopes

The vector balancing constant $\mathrm{vb}(K,Q)$ of two symmetric convex bodies $K,Q$ is the minimum $r \geq 0$ so that any number of vectors from $K$ can be balanced into an $r$-scaling of $Q$. A question raised by Schechtman is whether for any zonotope $K \subseteq \mathbb{R}^d$ one has $\mathrm{vb}(K,K) \lesssim \sqrt{d}$. Intuitively, this asks whether a natural geometric generalization of Spencer's Theorem (for which $K = B^d_\infty$) holds. We prove that for any zonotope $K \subseteq \mathbb{R}^d$ one has $\mathrm{vb}(K,K) \lesssim \sqrt{d} \log \log \log d$. Our main technical contribution is a tight lower bound on the Gaussian measure of any section of a normalized zonotope, generalizing Vaaler's Theorem for cubes. We also prove that for two different normalized zonotopes $K$ and $Q$ one has $\mathrm{vb}(K,Q) \lesssim \sqrt{d \log d}$. All the bounds are constructive and the corresponding colorings can be computed in polynomial time.

==> Makefile <==
MAIN = vectorBalancingConstantOfZonotopes
SOURCES = 

PAPER = letter

LATEX = latex
#BIBTEX = bibtex8 -W
BIBTEX = bibtex
DVIPS = dvips -f -Pcmz -G0 -t$(PAPER)
PSTOPDF = ps2pdf -dPDFsettings=/prepress -dAutoFilterColorImages=false \
  -dColorImageFilter=/FlateEncode
THUMBPDF = thumbpdf

ps: $(MAIN).ps

pdf: $(MAIN).pdf

$(MAIN).ps: $(MAIN).tex $(SOURCES)
#	$(LATEX) $(MAIN).tex
#	$(BIBTEX) $(MAIN)
	$(LATEX) $(MAIN).tex
	$(LATEX) $(MAIN).tex
	$(DVIPS) -o $(MAIN).ps $(MAIN).dvi

$(MAIN).pdf: $(MAIN).tex $(SOURCES)
	make ps
	$(PSTOPDF) $(MAIN).ps
	$(THUMBPDF) $(MAIN).pdf
	make ps
	$(PSTOPDF) $(MAIN).ps

clean:
	rm -rf $(MAIN).aux $(MAIN).dvi $(MAIN).log $(MAIN).blg $(MAIN).out *~

cleanall: clean
	rm -rf $(MAIN).bbl $(MAIN).ps $(MAIN).pdf

latexmk:
	latexmk -f -pdfps $(MAIN).tex

thomas:
	latexmk -f -pdfps $(MAIN).tex
	cp $(MAIN).pdf ~/Dropbox/CompiledPDFs/$(MAIN).pdf
	cp $(MAIN).tex ~/Dropbox/Backup/TexFiles/$(MAIN).tex
#	/Applications/Adobe\ Reader.app/Contents/MacOS/AdobeReader $(MAIN).pdf &
#	/Applications/Adobe\ Acrobat\ Reader\ DC.app/Contents/MacOS/AdobeReader $(MAIN).pdf &
	/Applications/Adobe\ Acrobat\ Reader.app/Contents/MacOS/AdobeReader $(MAIN).pdf &

all:
	make cleanall
	make pdf


